Sum-of-squares lower bounds for Non-Gaussian Component Analysis

Non-Gaussian Component Analysis (NGCA) is the statistical task of finding a non-Gaussian direction in a high-dimensional dataset. Specifically, given i.i.d.\ samples from a distribution $P^A_{v}$ on $\mathbb{R}^n$ that behaves like a known distribution $A$ in a hidden direction $v$ and like a standard Gaussian in the orthogonal complement, the goal is to approximate the hidden direction. The standard formulation posits that the first $k-1$ moments of $A$ match those of the standard Gaussian and the $k$-th moment differs. Under mild assumptions, this problem has sample complexity $O(n)$. On the other hand, all known efficient algorithms require $\Omega(n^{k/2})$ samples. Prior work developed sharp Statistical Query and low-degree testing lower bounds suggesting an information-computation tradeoff for this problem. Here we study the complexity of NGCA in the Sum-of-Squares (SoS) framework. Our main contribution is the first super-constant degree SoS lower bound for NGCA. Specifically, we show that if the non-Gaussian distribution $A$ matches the first $(k-1)$ moments of $\mathcal{N}(0, 1)$ and satisfies other mild conditions, then with fewer than $n^{(1 - \varepsilon)k/2}$ many samples from the normal distribution, with high probability, degree $(\log n)^{{1\over 2}-o_n(1)}$ SoS fails to refute the existence of such a direction $v$. Our result significantly strengthens prior work by establishing a super-polynomial information-computation tradeoff against a broader family of algorithms. As corollaries, we obtain SoS lower bounds for several problems in robust statistics and the learning of mixture models. Our SoS lower bound proof introduces a novel technique, that we believe may be of broader interest, and a number of refinements over existing methods.

==> prior_work.tex <==
\subsection{Prior Work}\label{sec: prior work}

Given the extensive literature on robust regression, here we focus on the most relevant work. 

\paragraph{GLM regression} 
{Various formalizations of} GLM regression 
{have} been studied extensively {over the past decades}; 
see., e,g., \citet{nelder1972generalized, kalai2009isotron, kakade2011efficient, klivans2017learning}. 
Recently, there has been increased focus on GLM regression {for activation functions that are popular in deep learning, including $\relu$s}. 
This problem has previously been considered both in the context of weaker noise models, 
such as the realizable/\new{random additive noise} setting ~\citep{Mahdi17, kalan2019fitting,yehudai2020learning}, 
as well as for more challenging noise models, 
\new{including adversarial label noise}~\citep{GoelKK19, DKZ20-sq-reg, GGK20, DKP21-SQ, DGKKS20, DKMR22, DKTZ22, WZDD23}. 

Even in the realizable setting \new{(i.e., with clean labels)}, 
it turns out that the squared loss has exponentially many local minima 
for the logistic activation function~\citep{Auer95}.
On the positive side,~\citet{DGKKS20} gave an efficient learner 
\new{achieving a constant factor approximation} 
{in the presence of adversarial label noise} 
under isotropic logconcave distributions. 
{This algorithmic result was 
generalized to broader families of activations under much milder distributional assumptions in~\citet{DKTZ22, WZDD23}.}
On the other hand, without distributional assumptions, 
even approximate learning is \new{computationally} hard~\citep{HardtM13, MR18, DKMR22}. 
{In a related direction, the problem has been studied in 
the distribution-free setting under semi-random label noise.}
%settings that are still challenging and making minimal assumptions about the input 
%while circumventing these computational hardness results. 
Specifically,~\citet{diakonikolas2021relu} focused on the setting 
of bounded (Massart) noise, where the adversary can arbitrarily corrupt 
a randomly selected subset of at most half the samples.
Even earlier,~\citet{karmakar2020study} studied the realizable setting 
under a noise model similar to (but more restrictive than) the Massart noise model, while~\citet{chen2020classification} studied a classification version of learning 
GLMs with Massart noise. 

In our work, we study the problem of \new{distribution-free learning of general GLMs 
in the presence of oblivious noise}, 
with the goal of being able to tolerate $1-o(1)$ fraction of the samples being corrupted.
In this setting, we recover the candidate solution 
to arbitrarily small precision in $\ell_1$ norm {(with respect to the objective}). 
Since $\norm{x}_2 \leq 1$ and $\norm{w}_2 \leq R$, it is easy to also provide the corresponding guarantees in the $\ell_2$ norm, which was the convention in \new{some earlier} works \citep{kakade2011efficient, GoelKK19}. 


\new{\paragraph{Algorithmic Robust Statistics}
A long line of work, initiated in~\cite{DKKLMS16, LaiRV16}, has focused on designing robust estimators
for a range of learning tasks (both supervised and unsupervised)
in the presence of a small constant fraction of adversarial corruptions; see~\cite{DiaKan22-book} for a textbook overview of this field. In the supervised setting, the underlying contamination model allows for corruptions in both $x$ and $y$ and makes no further assumptions on the power of the adversary. 
A limitation of these results is the assumption that the good data 
comes from a well-behaved distribution. 
On the other hand, without distributional assumptions on the clean data, these problems become computationally intractable. This fact motivates the study of weaker --- but still realistic --- noise models in which efficient noise-tolerant algorithms are possible in the distribution-free setting.
}


\new{\paragraph{Adversarial Label Corruptions}

In addition to adversarial corruptions in both $x$ and $y$, the adversarial label corruption model is another model which has been extensively studied in the context of linear and polynomial regression problems 
\cite{laska2009exact, Li2011CompressedSA, BhatiaJK15, BhatiaJKK17, kkp17, KarmalkarP19}. 
These results make strong assumptions on the distribution over the marginals. In contrast, we make no assumptions beyond the marginals coming from a bounded norm distribution.}



\paragraph{The Oblivious Noise Model} 
The oblivious noise model could be viewed as an attempt 
at characterizing the most general noise model 
that allows almost all points to be arbitrarily corrupted, 
while still allowing for recovery of the target function with vanishing error. 
This model has been considered for natural statistical problems, 
including PCA, sparse recovery~\citep{pesme2020online, d2021consistent}, 
as well as linear regression in the online setting~\citep{dalalyan2019outlier} and the problem of estimating a signal $x^*$ with additive oblivious noise~\citep{SoSOblivious21}.

The setting closest to the one considered in this paper is that of linear regression. Until very recently, the problem had
been studied primarily in the context of Gaussian design matrices, 
i.e., when $x$'s are drawn from $\cN(0, \Sigma)$. 
One of the main goals in this line of work is to design an algorithm 
that can tolerate the largest possible fraction of the labels being corrupted.
Initial works on linear regression either were not consistent as the error did 
not go to $0$ with increasing samples ~\citep{wright2008dense, NTN11} 
or failed to achieve the right convergence rates or breakdown point~\citep{Tsakonas14, BhatiaJK15}. \citet{suggala2019adaptive} provided the first consistent estimator 
achieving an error of $O(d/\alpha^2 m)$ for any $\alpha > 1/\log \log(m)$. 
Later, \citet{Steurer21Outliers} improved this rate to $\alpha > 1/d^c$ for constant $c$, while also generalizing the class of design matrices. 

Most of these prior results focused on either the oblivious noise 
being symmetric (or median $0$), or the underlying distribution being {(sub)-}Gaussian. 
In some of these settings (such as that of linear regression) 
it is possible to reduce the general problem 
to this restrictive setting, as is done in~\citet{norman2022robust}. 
However, for GLM regression, we cannot exploit the symmetry that is either induced by the distribution or the class of linear functions. 
In terms of lower bounds,~\citet{HT22} identify a ``well-spreadness'' condition (the column space of the measurements being far from sparse vectors) 
as a property that is necessary for recovery even when the oblivious noise is symmetric. 
Notably, these lower bounds are relevant when the goal is to perform parameter recovery or achieve a rate better than $\sigma^2/m$. 
In our paper, we instead give the first result for a far more general problem and with the objective of minimizing the clean loss, but not necessarily parameter recovery. 
Our lower bound follows from the fact that 
we cannot distinguish between translations of the target function from the data without making any assumptions on the oblivious noise. 



